Elastic weight consolidation for better bias inoculation

The biases present in training datasets have been shown to affect models for sentence pair classification tasks such as natural language inference (NLI) and fact verification. While fine-tuning models on additional data has been used to mitigate them, a common issue is that of catastrophic forgetting of the original training dataset. In this paper, we show that elastic weight consolidation (EWC) allows fine-tuning of models to mitigate biases while being less susceptible to catastrophic forgetting. In our evaluation on fact verification and NLI stress tests, we show that fine-tuning with EWC dominates standard fine-tuning, yielding models with lower levels of forgetting on the original (biased) dataset for equivalent gains in accuracy on the fine-tuning (unbiased) dataset.

==> graph_data_ablation.tex <==

\subsection{Data ablation}
\begin{figure}[H]
\centering
\begin{tikzpicture}
    \begin{axis}[
            xmin=25, xmax=700,
            ymin=0.75, ymax=0.95,
            width=7.5cm, height=4cm,
            grid = major,
            grid style={dashed, gray!30},
            ylabel=Accuracy,
            xlabel={Number of Training data},
            legend style={font=\footnotesize, at={(-0.0,-0.45)}, anchor=north west},
            legend columns=3
         ]
         
 
          
          \addplot [color=red, thick] table [skip first, x=num_train, y={avg model=roberta_base ewc=no}, col sep=comma] {data/CSV_Finetune_Ablation.csv};
          \addplot [color=orange, thick] table [skip first, x=num_train, y={avg model=roberta_base ewc=10000000}, col sep=comma] {data/CSV_Finetune_Ablation.csv};
          \addplot [color=olive, thick] table [skip first, x=max_instances, y={avg sym roberta_base l2}, col sep=comma] {data/CSV_L2_Finetune_Ablation.csv};
          \addplot [color=red, thick, dashed] table [skip first, x=max_instances, y={avg test fever noewc}, col sep=comma] {data/CSV_Finetune_FEVER.csv};
          \addplot [color=orange, thick, dashed] table [skip first, x=max_instances, y={avg test fever ewc}, col sep=comma] {data/CSV_Finetune_FEVER.csv};
          \addplot [color=olive, thick, dashed] table [skip first, x=max_instances, y={avg test roberta_base l2}, col sep=comma] {data/CSV_L2_Finetune_Ablation.csv};
          
          \legend{FT, FT+EWC, FT+L2}
    \end{axis}
    
    \end{tikzpicture}
    
    \caption{Data ablation when fine tuning RoBERTa FEVER model using the symmetric data. Solid lines indicate accuracy on symmetric test set. Dashed lines indicate accuracy on FEVER}
\end{figure}



==> table_2_old.tex <==

\begin{table*}[h]
\footnotesize
\begin{tabular}{lllllllll}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{4}{c}{\textbf{FEVER}}                                                                                  & \multicolumn{4}{c}{\textbf{Symmetric}}                                                                              \\ 
\cmidrule(l){2-5}
\cmidrule(l){6-9}
\multicolumn{1}{c}{}                                & \multicolumn{1}{c}{\textbf{Control}} &
\multicolumn{1}{c}{\textbf{Concat}} & \multicolumn{1}{c}{\textbf{FineTuned}} & \multicolumn{1}{c}{\textbf{FT+EWC}} & \multicolumn{1}{c}{\textbf{Control}} & \multicolumn{1}{c}{\textbf{Concat}} & \multicolumn{1}{c}{\textbf{FineTuned}} & \multicolumn{1}{c}{\textbf{FT+EWC}} \\ \toprule
ESIM+GloVe    & $79.97 \pm 0.4$   &   $79.57 \pm 0.4$   &   $70.78 \pm 1.1$   &   $74.64* \pm 0.7$   &   $68.37 \pm 1.0$   & $69.35 \pm 0.5$ & $74.21 \pm 1.3$   &   $73.20* \pm 1.4$ \\
ESIM+ELMo     & $80.15 \pm 0.2$   &   $80.33 \pm 0.8$   &   $76.45 \pm 0.8$   &   $78.09* \pm 0.4$   &   $64.04 \pm 0.7$   & $66.46 \pm 1.3$ & $68.68 \pm 0.7$   &   $69.16* \pm 0.7$ \\
BERT Base     & $86.88 \pm 0.5$   &   $86.87 \pm 0.5$   &   $78.82 \pm 0.9$   &   $82.23* \pm 1.1$   &   $74.77 \pm 1.4$   & $79.24 \pm 0.7$ & $87.07 \pm 0.6$   &   $85.11* \pm 0.4$ \\
RoBERTa Base  & $88.12 \pm 0.3$   &   $88.11 \pm 0.1$   &   $82.51 \pm 1.5$   &   $85.12* \pm 1.1$   &   $78.34 \pm 0.2$   & $87.03 \pm 2.3$ & $91.01 \pm 0.6$   &   $89.63* \pm 1.3$ \\ \bottomrule
\end{tabular}

\caption{Fine tuning FEVER NLI classifiers with symmetric data without (FineTuned column) and with (FT+EWC) elastic weight consolidation. For the FEVER columns. The values marked with * are reported at $p<0.01$ with a $t$-test compared to the FineTuned column. For the Symmetric column, the significance test is performed w.r.t the control column. \label{tab:test} }

\end{table*}

==> table_finetuning.tex <==
\begin{table*}[h]
\begin{tabular}{lllllll}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{3}{c}{\textbf{FEVER}}                                                                                  & \multicolumn{3}{c}{\textbf{Symmetric}}                                                                              \\ 
\cmidrule(l){2-4}
\cmidrule(l){5-7}
\multicolumn{1}{c}{}                                & \multicolumn{1}{c}{\textbf{Control}} & \multicolumn{1}{c}{\textbf{FineTuned}} & \multicolumn{1}{c}{\textbf{FT+EWC}} & \multicolumn{1}{c}{\textbf{Control}} & \multicolumn{1}{c}{\textbf{FineTuned}} & \multicolumn{1}{c}{\textbf{FT+EWC}} \\ \toprule
ESIM+GloVe  & 79.97 \pm 0.4 & 70.78 \pm 1.1 & 74.64* \pm 0.7 & 68.37 \pm 1.0 & 74.21 \pm  1.3 & 73.20* \pm 1.4 \\
ESIM+ELMo & 80.15 \pm 0.2 & 76.45 \pm 0.8 & 78.09* \pm 0.4  & 64.04 \pm 0.7 & 68.68 \pm 0.7 & 69.16* \pm 0.7 \\
BERT Base & 86.88 \pm 0.5 & 78.82 \pm 0.9 & 82.23* \pm 1.1 & 74.77 \pm 1.4 & 87.07 \pm 0.6 & 85.11* \pm 0.4 \\
RoBERTa Base & 88.12 \pm 0.3 & 82.51 \pm 1.5 & 85.12* \pm 1.1 & 78.34 \pm 0.2 & 91.01 \pm 0.6 & 89.63* \pm 1.3  \\ \bottomrule
\end{tabular}

\caption{Fine tuning FEVER NLI classifiers with symmetric data without (FineTuned column) and with (FT+EWC) elastic weight consolidation. For the FEVER columns. The values marked with * are reported at $p<0.01$ with a $t$-test compared to the FineTuned column. For the Symmetric column, the significance test is performed w.r.t the control column. \label{tab:test} }

\end{table*}
